Accelerating Guided Diffusion Sampling with Splitting Numerical Methods

Guided diffusion is a technique for conditioning the output of a diffusion model at sampling time without retraining the network for each specific task. One drawback of diffusion models, however, is their slow sampling process. Recent techniques can accelerate unguided sampling by applying high-order numerical methods to the sampling process when viewed as differential equations. On the contrary, we discover that the same techniques do not work for guided sampling, and little has been explored about its acceleration. This paper explores the culprit of this problem and provides a solution based on operator splitting methods, motivated by our key finding that classical high-order numerical methods are unsuitable for the conditional function. Our proposed method can re-utilize the high-order methods for guided sampling and can generate images with the same quality as a 250-step DDIM baseline using 32-58% less sampling time on ImageNet256. We also demonstrate usage on a wide variety of conditional generation tasks, such as text-to-image generation, colorization, inpainting, and super-resolution.

==> content/1Intro.tex <==
\section{Introduction}
A family of generative models known as diffusion models has recently gained a lot of attention with state-of-the-art image generation quality \citep{dhariwal2021diffusion}.
%When compared to the widely used generative adversarial networks (GANs) \citep{goodfellow2014generative}, the diffusion models have shown competitive image quality \citep{dhariwal2021diffusion}.
\emph{Guided diffusion} is an approach for controlling the output of a trained diffusion model for conditional generation tasks without retraining its network.
%by modifying only the sampling procedure.
By engineering a task-specific conditional function and modifying only the sampling procedure, guided diffusion models can be used in a variety of applications, such as class-conditional image generation \citep{dhariwal2021diffusion,kawar2022enhancing}, text-to-image generation \citep{nichol2021glide}, image-to-image translation \citep{zhao2022egsde}, inpainting \citep{chung2022improving}, colorization \citep{song2020score}, image composition \citep{sasaki2021unit}, adversarial purification \citep{wang2022guided,wu2022guided} and super-resolution \citep{choi2021ilvr}.


One common drawback of both guided and regular ``unguided'' diffusion models is their slow sampling processes, usually requiring hundreds of iterations to produce a single image. 
Recent speed-up attempts include improving the noise schedule \citep{nichol2021improved,watson2021learning}, redefining the diffusion process to be non-Markovian, thereby allowing a deterministic sampling process \cite{song2020denoising}, network distillation that teaches a student model to simulate multiple sampling steps of a teacher model \cite{salimans2022progressive, luhman2021knowledge}, among others. \cite{song2020denoising} show how each sampling step can be expressed as a first-order numerical step of an ordinary differential equation (ODE). Similarly, \cite{song2020score} express the sampling of a score-based model as solving a stochastic differential equation (SDE). By regarding the sampling process as an ODE/SDE, many high-order numerical methods have been suggested, such as \cite{liu2022pseudo}, \cite{zhang2022fast}, and \cite{zhang2022gddim} with impressive results on unguided diffusion models.
%This problem has spurred numerous studies in many directions, such as improving noise schedules \citep{nichol2021improved,watson2021learning} and network distillation \cite{salimans2022progressive, luhman2021knowledge}.
%Many research studies has focused on improving the diffusion sampling speed.
%\cite{song2020denoising} propose a deterministic sampler capable of producing high-quality results in fewer steps by redefining the diffusion process to be non-Markovian.
%capable of producing high-quality results with fewer steps.
%Each sampling step can be expressed as a first-order numerical step of an ordinary differential equation (ODE).
%Similarly, \cite{song2020score} show how diffusion sampling can be viewed as solving a stochastic differential equation (SDE).
%Many high-order numerical methods have been suggested specifically for the ODE/SDE, such as \cite{liu2022pseudo}, \cite{zhang2022fast}, and \cite{zhang2022gddim} with impressive results on unguided diffusion models.
%These methods produce very impressive results on unguided diffusion models.
However, when applied to guided diffusion models, these methods produce surprisingly poor results (see Figure \ref{fig:class})---given a few number of steps, those high-order numerical methods actually perform worse than low-order methods. 

Guided sampling differs from the unguided one by the addition of the gradients of the conditional function to its sampling equation. The observed performance decline thus suggests that classical high-order methods may not be suitable for the conditional function and, consequently, the guided sampling equation as a whole. Our paper tests this hypothesis and presents an approach to accelerating guided diffusion sampling.
The key idea is to use an \emph{operator splitting} method to split the less well-behaved conditional function term from the standard diffusion term and solve them separately. 
%that is already well suited to high-order methods. 
This approach not only allows re-utilizing the successful high-order methods on the diffusion term but also provides us with options to combine different specialized methods for each term to maximize performance. Splitting method can be used to solve diffusion SDE in \cite{dockhorn2021score}. %added
%to split the guided sampling equation into 
%Our key idea is to formulate guided sampling as an ODE with two terms where the first term contains standard diffusion gradients well suitable for high-order numerical methods, and the second contains the less well-behaved conditioning gradients. We can then solve the ODE using an \emph{operator splitting} method and separately choose a different order and type of numerical method for solving each term. This approach allows us to re-utilize high-order methods previously failed on guided sampling.   
%We hypothesis that the conditional term
%We observe that these gradients are the only term not suitable to high-order methods and that one can separately handle different terms, each with a different numerical behavior, through an \emph{operator splitting} method. 
%This paper 
%We hypothesize that the performance decline declined because the numerical method is chosen as inapplicable for the gradient term.
%We hypothesize that the performance decline is due to the behavior of the conditional function that is not suitable to high-order methods. 
%This paper presents an approach to accelerating guided diffusion sampling. The key idea is to formulate guided diffusion sampling as an ODE with two terms where the first term contains standard diffusion gradients well suitable for high-order numerical methods, and the second contains the less well-behaved conditioning gradients. We can then solve the ODE using an \emph{operator splitting} method and separately choose a different order and type of numerical method for solving each term. This approach allows us to re-utilize high-order methods previously failed on guided sampling.  
%select best splitting combining different numerical methods for each term with different splitting  with different combinations of splitting strategies and numerical methods of each term.
%This allows us 
%and bring back high-order numerical methods that had failed on guided diffusion models.

Our design process includes comparing different splitting methods and numerical methods for each split term.
%as well as selecting the best numerical scheme for each split part.
%Together, we can determine which numerical combination provides the best quality/speed tradeoff for the guided diffusion model.
%Our method outperforms all previous work 
When tested on ImageNet, our approach achieves the same level of image quality as a DDIM baseline while reducing the sampling time by approximately 32-58\%.
%With the same, fixed sampling time, our approach also provides better image quality as measured by LPIPS, FID, and Perception/Recall. 
Compared with other sampling methods using the same sampling time, our approach provides better image quality as measured by LPIPS, FID, and Perception/Recall. 
With only minimal modifications to the sampling equation, we also show successful acceleration on various conditional generation tasks.
%, such as text-to-image synthesis, image in-painting, colorization, and super-resolution
%, using no modifications to the training procedure.
%To show that our approach can be used for any guided diffusion without retraining, we apply it to various tasks, such as text-to-image synthesis, image in-painting, colorization, and super-resolution

\begin{figure*}
    \centering
    \setlength\tabcolsep{1.5pt}
    \begin{tabular}{cl}
    \shortstack{\small Number \\of steps} & \qquad\: 8 \qquad\qquad\: 16 \qquad\qquad 32 \qquad\qquad 64 \qquad\qquad 128 \qquad\quad 256  \\
    \shortstack{DDIM\vspace{0.8cm}} &
    \includegraphics[width=0.8\textwidth]{images/class_gen/v4/ddim_p.jpg} \\
    \shortstack{PLMS4\vspace{0.8cm}} &
    \includegraphics[width=0.8\textwidth]{images/class_gen/v4/plms_p.jpg}\\
    \shortstack{\textbf{STSP4}\\(Ours)\vspace{0.5cm}} &
    \includegraphics[width=0.8\textwidth]{images/class_gen/v4/bchf_p.jpg} \\
    \end{tabular}
    \caption{
    %We present an approach for accelerating guided diffusion sampling.
Generated samples of a classifier-guided diffusion model trained on ImageNet256 using 8-256 sampling steps from different sampling methods.
Our technique, STSP4, produces high-quality results in a fewer number of steps.
%has steady quality even when the number of steps is low, whereas other high-order methods show a fast decrease in performance when the number of steps is reduced.
    }
    \label{fig:class}
\end{figure*}

==> content/recycle/2general_format.tex <==
\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone, regardless of the formatter being used.

\subsection{Citations within the text}

Citations within the text should be based on the \texttt{natbib} package
and include the authors' last names and year (with the ``et~al.'' construct
for more than two authors). When the authors or the publication are
included in the sentence, the citation should not be in parenthesis using \verb|\citet{}| (as
in ``See \citet{Hinton06} for more information.''). Otherwise, the citation
should be in parenthesis using \verb|\citep{}| (as in ``Deep learning shows promise to make progress
towards AI~\citep{Bengio+chapter2007}.'').

The corresponding references are to be listed in alphabetical order of
authors, in the \textsc{References} section. As to the format of the
references themselves, any style is acceptable as long as it is used
consistently.

\subsection{Footnotes}

Indicate footnotes with a number\footnote{Sample of the first footnote} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches
(12~picas).\footnote{Sample of the second footnote}

\subsection{Figures}

All artwork must be neat, clean, and legible. Lines should be dark
enough for purposes of reproduction; art work should not be
hand-drawn. The figure number and caption always appear after the
figure. Place one line space before the figure caption, and one line
space after the figure. The figure caption is lower case (except for
first word and proper nouns); figures are numbered consecutively.

Make sure the figure caption does not get separated from the figure.
Leave sufficient space to avoid splitting the figure and figure caption.

You may use color figures.
However, it is best for the
figure captions and the paper body to make sense if the paper is printed
either in black/white or in color.
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\end{center}
\caption{Sample figure caption.}
\end{figure}

\subsection{Tables}

All tables must be centered, neat, clean and legible. Do not use hand-drawn
tables. The table number and title always appear before the table. See
Table~\ref{sample-table}.

Place one line space before the table title, one line space after the table
title, and one line space after the table. The table title must be lower case
(except for first word and proper nouns); tables are numbered consecutively.

\begin{table}[t]
\caption{Sample table title}
\label{sample-table}
\begin{center}
\begin{tabular}{ll}
\multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
\\ \hline \\
Dendrite         &Input terminal \\
Axon             &Output terminal \\
Soma             &Cell body (contains cell nucleus) \\
\end{tabular}
\end{center}
\end{table}

==> content/recycle/3others.tex <==
\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}



\section{Final instructions}
Do not change any aspects of the formatting parameters in the style files.
In particular, do not modify the width or length of the rectangle the text
should fit into, and do not change font sizes (except perhaps in the
\textsc{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PostScript or PDF files}

Please prepare PostScript or PDF files with paper size ``US Letter'', and
not, for example, ``A4''. The -t
letter option on dvips will produce US Letter files.

Consider directly generating PDF files using \verb+pdflatex+
(especially if you are a MiKTeX user).
PDF figures must be substituted for EPS figures, however.

Otherwise, please generate your PostScript and PDF files with the following commands:
\begin{verbatim}
dvips mypaper.dvi -t letter -Ppdf -G0 -o mypaper.ps
ps2pdf mypaper.ps mypaper.pdf
\end{verbatim}

\subsection{Margins in LaTeX}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+
from the graphicx package. Always specify the figure width as a multiple of
the line width as in the example below using .eps graphics
\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.eps}
\end{verbatim}
or % Apr 2009 addition
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
for .pdf graphics.
See section~4.4 in the graphics bundle documentation (\url{http://www.ctan.org/tex-archive/macros/latex/required/graphics/grfguide.ps})

A number of width problems arise when LaTeX cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command.

\subsubsection*{Author Contributions}
If you'd like to, you may include  a section for author contributions as is done
in many journals. This is optional and at the discretion of the authors.

\subsubsection*{Acknowledgments}
Use unnumbered third level headings for the acknowledgments. All
acknowledgments, including those to funding agencies, go at the end of the paper.

==> content/recycle/4_1figure_backup.tex <==
\begin{table}
  \begin{minipage}{0.5\columnwidth}
    \centering
    \resizebox{0.98\columnwidth}{!}{
    \begin{tabular}{lccccc}
        \toprule
        Method & Steps & FID  & sFID & Prec & Rec \\
        \midrule
        \multicolumn{4}{l}{\textbf{ImageNet128}} \\
        \arrayrulecolor[rgb]{0.7, 0.7, 0.7}\hline
       \rule{0pt}{2ex}DDIM             & 25   & 6.69 & 7.77 & 0.78    & 0.49 \\
       PLMS2            & 25   & 5.71 & 6.39 & 0.80    & 0.51 \\
       PLMS4            & 25   & 4.97 & 5.76 & 0.80    & 0.53 \\
       \textbf{LTSP2}   & 25   & 5.14 & 6.33 & 0.81    & 0.51 \\
       \textbf{LTSP4}   & 25   & 3.85 & \textbf{5.15} &\textbf{0.81} & \textbf{0.54} \\
       \textbf{STSP2}   & 20   & 5.33 & 6.59 & 0.80    & 0.52 \\
       \textbf{STSP4}   & 20   &\textbf{3.78}& 5.23& \textbf{0.81}& \textbf{0.54} \\
       [-1.2em]\\
       \hdashline[1.2pt/1.2pt]\arrayrulecolor{black}
       \rule{0pt}{2ex}\textit{ADM-G}  & \textit{250} & \textit{2.97} & \textit{5.09} & \textit{0.78}  & \textit{0.59} \\
       \bottomrule
       \\
       [-0.2em]\\
    \end{tabular}}
  \end{minipage}\hfill 
  \begin{minipage}{0.5\columnwidth}
    \centering
    \resizebox{0.98\columnwidth}{!}{
    \begin{tabular}{lccccc}
        %\hline
        \toprule
        Method & Steps & FID & sFID & Prec & Rec \\
        \midrule
        \multicolumn{4}{l}{\textbf{ImageNet256}} \\
        \arrayrulecolor[rgb]{0.7, 0.7, 0.7}\hline
       \rule{0pt}{2ex}DDIM             & 25   & 5.47 & 5.69 & 0.80    & 0.47 \\
       PLMS4            & 25   & 4.71 & 5.13 & 0.82    & 0.49 \\
       \textbf{STSP4}   & 20   &\textbf{4.49}&\textbf{5.05}& \textbf{0.83}& \textbf{0.50} \\
       [-1.2em]\\
       \hdashline[1.2pt/1.2pt]\arrayrulecolor{black}
       \rule{0pt}{2ex}\textit{ADM-G}   & \textit{250}     & \textit{4.59} & \textit{5.25} & \textit{0.82}     & \textit{0.50} \\
        \\
        \multicolumn{4}{l}{\textbf{ImageNet512}} \\
        \arrayrulecolor[rgb]{0.7, 0.7, 0.7}\hline
       \rule{0pt}{2ex}DDIM             & 25   & 9.07 & 13.18 & {0.81}    & 0.42 \\
       PLMS4            & 25   & 16.00 & \textbf{8.22} & {0.75}    & \textbf{0.51} \\
       \textbf{STSP4}   & 20   &\textbf{8.24}&{9.95}& \textbf{0.83}& {0.45} \\
       [-1.2em]\\
       \hdashline[1.2pt/1.2pt]\arrayrulecolor{black}
       \rule{0pt}{2ex}\textit{ADM-G}   & \textit{250}  & \textit{7.72} & \textit{6.57} & \textit{0.87}     & \textit{0.42} \\
       \bottomrule
    \end{tabular}}
  \end{minipage}
    \caption{Quality comparison for classifier-guided condition image generation on ImageNet. The bold method name mean our propose methods. The best score in each measurement are represent by bold.  20-step of STSP still have a shorter evaluation time than DDIM in 25 steps in every case.  We provide the reported score from \cite{dhariwal2021diffusion} using 250 sampling steps, referred to as ADM-G in their paper.}
    \label{tab:Sampling}
\end{table}

==> content/recycle/5_1figure.tex <==


\begin{figure*}
    \centering
    \setlength\tabcolsep{1.5pt}
    \begin{tabular}{ccccc}
        \includegraphics[width=0.125\textwidth]{images/inpainting/task2/gt.png}
        \includegraphics[width=0.25\textwidth]{images/inpainting/task2/ddim.png}
        \includegraphics[width=0.25\textwidth]{images/inpainting/task2/ltts.png}
        \includegraphics[width=0.25\textwidth]{images/inpainting/task2/bchf.png}
        \\
        \shortstack{
         \includegraphics[width=0.125\textwidth]{images/inpainting/task1/gt.png}
         \\  input}
         \shortstack{
         \includegraphics[width=0.25\textwidth]{images/inpainting/task1/ddim.png}
         \\  DDIM}
         \shortstack{
         \includegraphics[width=0.25\textwidth]{images/inpainting/task1/ltts.png}
         \\  LTTS1}
         \shortstack{
         \includegraphics[width=0.25\textwidth]{images/inpainting/task1/bchf.png}
         \\  BCHF4}
    \end{tabular}
    \caption{inpainting with 50 steps
    }
    \label{fig_inpaint}
\end{figure*}


\begin{figure*}
    \centering
    \setlength\tabcolsep{1.5pt}
    \begin{tabular}{ccccc}
        \includegraphics[width=0.125\textwidth]{images/colorization/task2/gt.png}
        \includegraphics[width=0.25\textwidth]{images/colorization/task2/ddim.png}
        \includegraphics[width=0.25\textwidth]{images/colorization/task2/ltts.png}
        \includegraphics[width=0.25\textwidth]{images/colorization/task2/bchf.png}
        \\
        \shortstack{
         \includegraphics[width=0.125\textwidth]{images/colorization/task1/gt.png}
         \\  input}
         \shortstack{
         \includegraphics[width=0.25\textwidth]{images/colorization/task1/ddim.png}
         \\  DDIM}
         \shortstack{
         \includegraphics[width=0.25\textwidth]{images/colorization/task1/ltts.png}
         \\  LTTS1}
         \shortstack{
         \includegraphics[width=0.25\textwidth]{images/colorization/task1/bchf.png}
         \\  BCHF4}
    \end{tabular}
    \caption{colorization with 50 steps
    }
    \label{fig_color}
\end{figure*}


\begin{figure*}
    \centering
    \setlength\tabcolsep{1.5pt}
    \begin{tabular}{ccccc}
        \includegraphics[width=0.125\textwidth]{images/super/task2/gt.png}
        \includegraphics[width=0.25\textwidth]{images/super/task2/ddim.png}
        \includegraphics[width=0.25\textwidth]{images/super/task2/ltts.png}
        \includegraphics[width=0.25\textwidth]{images/super/task2/bchf.png}
        \\
        \shortstack{
         \includegraphics[width=0.125\textwidth]{images/super/task1/gt.png}
         \\  input}
         \shortstack{
         \includegraphics[width=0.25\textwidth]{images/super/task1/ddim.png}
         \\  DDIM}
         \shortstack{
         \includegraphics[width=0.25\textwidth]{images/super/task1/ltts.png}
         \\  LTTS1}
         \shortstack{
         \includegraphics[width=0.25\textwidth]{images/super/task1/bchf.png}
         \\  BCHF4}
    \end{tabular}
    \caption{8x super-resoltuion with 50 steps
    }
    \label{fig_super}
\end{figure*}

==> content/recycle/5_3figure.tex <==
\begin{figure*}
    \centering
    \setlength\tabcolsep{1.5pt}
    \begin{tabular}{cc|c|c@{}c@{}c|ccc}
        &Original & Input & &STSP4& & & DDIM \\
        \parbox[t]{2mm}{\rotatebox{90}{Inpainting}}&
        \shortstack{
            \includegraphics[width=0.11\textwidth]{images/inpainting/task3/gt.png} \\
            \includegraphics[width=0.11\textwidth]{images/inpainting/task4/gt.png} } &
        \shortstack{
            \includegraphics[width=0.11\textwidth]{images/inpainting/task3/input.png} \\
            \includegraphics[width=0.11\textwidth]{images/inpainting/task4/input.png} } &
        \shortstack{
            \includegraphics[width=0.11\textwidth]{images/inpainting/task3/bchf1.png} \\
            \includegraphics[width=0.11\textwidth]{images/inpainting/task4/bchf1.png} } &
        \shortstack{
            \includegraphics[width=0.11\textwidth]{images/inpainting/task3/bchf2.png} \\
            \includegraphics[width=0.11\textwidth]{images/inpainting/task4/bchf2.png} } &
        \shortstack{
            \includegraphics[width=0.11\textwidth]{images/inpainting/task3/bchf3.png} \\
            \includegraphics[width=0.11\textwidth]{images/inpainting/task4/bchf3.png} } \\
        \hline  
        \rotatebox{90}{Colorization}&
        \includegraphics[width=0.11\textwidth]{images/colorization/task3/gt.png} &
        \includegraphics[width=0.11\textwidth]{images/colorization/task3/input.png}&
        \includegraphics[width=0.11\textwidth]{images/colorization/task3/bchf1.png}&
        \includegraphics[width=0.11\textwidth]{images/colorization/task3/bchf2.png}&
        \includegraphics[width=0.11\textwidth]{images/colorization/task3/bchf3.png}&
        \includegraphics[width=0.11\textwidth]{images/colorization/task3/ddim1.png}&
        \includegraphics[width=0.11\textwidth]{images/colorization/task3/ddim2.png}&
        \includegraphics[width=0.11\textwidth]{images/colorization/task3/ddim3.png} \\&
        \includegraphics[width=0.11\textwidth]{images/colorization/task4/gt.png} &
        \includegraphics[width=0.11\textwidth]{images/colorization/task4/input.png}&
        \includegraphics[width=0.11\textwidth]{images/colorization/task4/bchf1.png}&
        \includegraphics[width=0.11\textwidth]{images/colorization/task4/bchf2.png}&
        \includegraphics[width=0.11\textwidth]{images/colorization/task4/bchf3.png}&
        \includegraphics[width=0.11\textwidth]{images/colorization/task4/ddim1.png}&
        \includegraphics[width=0.11\textwidth]{images/colorization/task4/ddim2.png}&
        \includegraphics[width=0.11\textwidth]{images/colorization/task4/ddim3.png} \\
        \hline  
        \rotatebox{90}{Super-Resolution}&
        \includegraphics[width=0.11\textwidth]{images/super/task3/gt.png} &
        \includegraphics[width=0.11\textwidth]{images/super/task3/input.png}&
        \includegraphics[width=0.11\textwidth]{images/super/task3/bchf1.png}&
        \includegraphics[width=0.11\textwidth]{images/super/task3/bchf2.png}&
        \includegraphics[width=0.11\textwidth]{images/super/task3/bchf3.png}&
        \includegraphics[width=0.11\textwidth]{images/super/task3/ddim1.png}&
        \includegraphics[width=0.11\textwidth]{images/super/task3/ddim2.png}&
        \includegraphics[width=0.11\textwidth]{images/super/task3/ddim3.png}\\&
        \includegraphics[width=0.11\textwidth]{images/super/task4/gt.png} &
        \includegraphics[width=0.11\textwidth]{images/super/task4/input.png}&
        \includegraphics[width=0.11\textwidth]{images/super/task4/bchf1.png}&
        \includegraphics[width=0.11\textwidth]{images/super/task4/bchf2.png}&
        \includegraphics[width=0.11\textwidth]{images/super/task4/bchf3.png}&
        \includegraphics[width=0.11\textwidth]{images/super/task4/ddim1.png}&
        \includegraphics[width=0.11\textwidth]{images/super/task4/ddim2.png}&
        \includegraphics[width=0.11\textwidth]{images/super/task4/ddim3.png}
    \end{tabular}
    \caption{inpainting with 30 steps
    }
    \label{fig_inpaint}
\end{figure*}
